On the Reconstruction of Geodesic Subspaces of $\mathbb{R}^N$

We consider the topological and geometric reconstruction of a geodesic subspace of $\mathbb{R}^N$ both from the \v{C}ech and Vietoris-Rips filtrations on a finite, Hausdorff-close, Euclidean sample. Our reconstruction technique leverages the intrinsic length metric induced by the geodesics on the subspace. We consider the distortion and convexity radius as our sampling parameters for a successful reconstruction. For a geodesic subspace with finite distortion and positive convexity radius, we guarantee a correct computation of its homotopy and homology groups from the sample. For geodesic subspaces of $\mathbb{R}^2$, we also devise an algorithm to output a homotopy equivalent geometric complex that has a very small Hausdorff distance to the unknown shape of interest.

==> Figures/nerve.tex <==
\begin{tikzpicture}[scale=1.0]
  %% Define the vertices
  \coordinate (v1) at (0,0);
  \coordinate (v2) at (-2,-3);
  \coordinate (v3) at (1,3);
  \coordinate (v4) at (-4,-1);
  \coordinate (v5) at (1,0.5);
  \coordinate (v5) at (1,0.5);
  \coordinate (v6) at (3,-2);

  %% Define the sample points
  \coordinate (x1) at (barycentric cs:v1=0.5,v2=0.5);
  \coordinate (x2) at (barycentric cs:v1=0.25,v2=0.75);
  \coordinate (x3) at (barycentric cs:v1=0.72,v2=.28);

  \coordinate (x4) at (barycentric cs:v2=0.65,v4=0.35);
  \coordinate (x5) at (barycentric cs:v2=0.4,v4=.6);
  \coordinate (x6) at (barycentric cs:v2=0.05,v4=0.95);
  \coordinate (x7) at (barycentric cs:v2=0.9,v4=.1);

  \coordinate (x8) at  (barycentric cs:v1=0.25,v4=0.75);
  \coordinate (x9) at  (barycentric cs:v1=0.75,v4=.25);
  \coordinate (x10) at (barycentric cs:v1=0.5,v4=.5);

  \coordinate (x11) at (barycentric cs:v1=0.985,v3=0.015);
  \coordinate (x12) at (barycentric cs:v1=0.7,v3=0.3);
  \coordinate (x13) at (barycentric cs:v1=0.43,v3=0.57);
  \coordinate (x14) at (barycentric cs:v1=0.16,v3=0.84);

  \coordinate (x15) at (barycentric cs:v3=0.2,v5=0.8);

  \coordinate (x16) at (barycentric cs:v5=0.85,v6=0.15);
  \coordinate (x17) at (barycentric cs:v5=0.7,v6=0.3);
  \coordinate (x18) at (barycentric cs:v5=0.55,v6=0.45);
  \coordinate (x19) at (barycentric cs:v5=0.25,v6=0.75);
  \coordinate (x20) at (barycentric cs:v5=0.1,v6=0.9);

  \foreach \i in {1,...,20}{
    \draw[draw=gray!70,fill=gray!40,opacity=0.6] (x\i)
    circle (15pt);
    \draw[fill=black!50,opacity=0.5] (x\i)
    node[above,opacity=0.7,gray!70] {$x_{\i}$} circle (2pt);
  }

  \draw[red!60,ultra thick,opacity=0.6]
  (x1)  -- (x3)
  (x1)  -- (x2)
  (x2)  -- (x7)
  (x7)  -- (x4)
  (x4)  -- (x5)
  (x5)  -- (x6)
  (x5)  -- (x8)
  (x6)  -- (x8)
  (x8)  -- (x10)
  (x10) -- (x9)
  (x9)  -- (x3)
  (x9)  -- (x11)
  (x3)  -- (x11)
  (x11) -- (x12)
  (x12) -- (x15)
  (x12) -- (x13)
  (x13) -- (x15)
  (x13) -- (x14)
  (x15) -- (x16)
  (x16) -- (x17)
  (x17) -- (x18)
  (x16) to[bend right] (x18)
  (x18) -- (x19)
  (x19) -- (x20);

  \fill[fill=blue!20,opacity=0.5]
  (x12) -- (x13) -- (x15);

  \fill[fill=blue!20,opacity=0.5]
  (x16) -- (x17) -- (x18) to[bend left,bend angle=120] (x16);

\end{tikzpicture}


==> Figures/nerve_1.tex <==
\begin{tikzpicture}[scale=2.0]
  %% Define the vertices
  \coordinate (v1) at (0,0);
  \coordinate (v2) at (-2,-3);
  \coordinate (v3) at (1,3);
  \coordinate (v4) at (-4,-1);
  \coordinate (v5) at (1,0.5);
  \coordinate (v5) at (1,0.5);
  \coordinate (v6) at (3,-2);

  %% Define the sample points
  \coordinate (x1) at (barycentric cs:v1=0.5,v2=0.5);
  \coordinate (x2) at (barycentric cs:v1=0.25,v2=0.75);
  \coordinate (x3) at (barycentric cs:v1=0.72,v2=.28);

  \coordinate (x4) at (barycentric cs:v2=0.65,v4=0.35);
  \coordinate (x5) at (barycentric cs:v2=0.4,v4=.6);
  \coordinate (x6) at (barycentric cs:v2=0.05,v4=0.95);
  \coordinate (x7) at (barycentric cs:v2=0.9,v4=.1);

  \coordinate (x8) at  (barycentric cs:v1=0.25,v4=0.75);
  \coordinate (x9) at  (barycentric cs:v1=0.75,v4=.25);
  \coordinate (x10) at (barycentric cs:v1=0.5,v4=.5);

  \coordinate (x11) at (barycentric cs:v1=0.985,v3=0.015);
  \coordinate (x12) at (barycentric cs:v1=0.7,v3=0.3);
  \coordinate (x13) at (barycentric cs:v1=0.43,v3=0.57);
  \coordinate (x14) at (barycentric cs:v1=0.16,v3=0.84);

  \coordinate (x15) at (barycentric cs:v3=0.2,v5=0.8);

  \coordinate (x16) at (barycentric cs:v5=0.85,v6=0.15);
  \coordinate (x17) at (barycentric cs:v5=0.7,v6=0.3);
  \coordinate (x18) at (barycentric cs:v5=0.55,v6=0.45);
  \coordinate (x19) at (barycentric cs:v5=0.25,v6=0.75);
  \coordinate (x20) at (barycentric cs:v5=0.1,v6=0.9);

  \foreach \i in {1,...,20}{
    \draw[fill=black!50,opacity=0.7] (x\i)
    node[above,opacity=1,gray!90] {$x_{\i}$} circle (2pt);
  }

  \draw[red!60,ultra thick,opacity=0.8]
  (x1)  -- (x3)
  (x1)  -- (x2)
  (x2)  -- (x7)
  (x7)  -- (x4)
  (x4)  -- (x5)
  (x5)  -- (x6)
  (x5)  -- (x8)
  (x6)  -- (x8)
  (x8)  -- (x10)
  (x10) -- (x9)
  (x9)  -- (x3)
  (x9)  -- (x11)
  (x3)  -- (x11)
  (x11) -- (x12)
  (x12) -- (x15)
  (x12) -- (x13)
  (x13) -- (x15)
  (x13) -- (x14)
  (x15) -- (x16)
  (x16) -- (x17)
  (x17) -- (x18)
  (x16) to[bend right] (x18)
  (x18) -- (x19)
  (x19) -- (x20);

  \fill[fill=blue!20,opacity=0.7]
  (x12) -- (x13) -- (x15);

  \fill[fill=blue!20,opacity=0.7]
  (x16) -- (x17) -- (x18) to[bend left,bend angle=120] (x16);

\end{tikzpicture}


==> Figures/typical_graph.tex <==
\begin{tikzpicture}[scale=1.0]
  %% Define the vertices
  \coordinate (v1) at (0,0);
  \coordinate (v2) at (-2,-3);
  \coordinate (v3) at (1,3);
  \coordinate (v4) at (-4,-1);
  \coordinate (v5) at (1,0.5);
  \coordinate (v5) at (1,0.5);
  \coordinate (v6) at (3,-2);
  %% Draw the edges
  \path[edge]
  (v1) -- (v4)
  (v4) -- (v2)
  (v1) -- (v3)
  (v3) -- (v5)
  (v1) -- (v2)
  (v5) -- (v6);
  %% Draw the verticles
  \draw[vertex]
  (v1) node[anchor=west]  {$v_1$} circle (3pt)
  (v2) node[anchor=north] {$v_2$} circle (3pt)
  (v3) node[anchor=south] {$v_3$} circle (3pt)
  (v4) node[anchor=north] {$v_4$} circle (3pt)
  (v5) node[anchor=north] {$v_5$} circle (3pt)
  (v6) node[anchor=north] {$v_6$} circle (3pt);
\end{tikzpicture}
\caption{A typical planar metric graph}

